Reward Augmentation in Reinforcement Learning for Testing Distributed Systems

Bugs in popular distributed protocol implementations have been the source of many downtimes in popular internet services. We describe a randomized testing approach for distributed protocol implementations based on reinforcement learning. Since the natural reward structure is very sparse, the key to successful exploration in reinforcement learning is reward augmentation. We show two different techniques that build on one another. First, we provide a decaying exploration bonus based on the discovery of new states -- the reward decays as the same state is visited multiple times. The exploration bonus captures the intuition from coverage-guided fuzzing of prioritizing new coverage points; in contrast to other schemes, we show that taking the maximum of the bonus and the Q-value leads to more effective exploration. Second, we provide waypoints to the algorithm as a sequence of predicates that capture interesting semantic scenarios. Waypoints exploit designer insight about the protocol and guide the exploration to ``interesting'' parts of the state space. Our reward structure ensures that new episodes can reliably get to deep interesting states even without execution caching. We have implemented our algorithm in Go. Our evaluation on three large benchmarks (RedisRaft, Etcd, and RSL) shows that our algorithm can significantly outperform baseline approaches in terms of coverage and bug finding.

==> contents/predh_copy.tex <==
\begin{algorithm}
    \SetAlgoLined
    \SetKwInOut{Input}{Input}
    \SetKwProg{Def}{def}{:}{}
    \Input{$\alpha, \gamma, \epsilon, \left\{pred_1, \cdots, pred_n\right\}, oneTime \in \left\{\top, \bot\right\}$}
    \BlankLine

    $V_p(s,a) \gets 0$ for all $s \in \stateSpace, a \in \actionSpace, p \in pred_1, \cdots pred_n$\;
    \BlankLine

    \tcp{Reset the variables at the start of the iteration}
    \Def{$resetIteration()$}{
        $curPred \gets 1$\;
        $targetReached \gets \bot$\;
        $traceSegments \gets ()$
    }
    \BlankLine

    \Def{$pick(s, \left\{a_1, \cdots, a_k\right\})$}{
        \If{$rand(0,1) < \epsilon$}{
            \Return{$a_{rand(1,k)}$}
        }
        \Else{
            \Return{$arg \max_{a \in \left\{a_1, \cdots, a_k\right\}} Q_{curPred}(s,a,1)$}
        }
    }
    \BlankLine

    \tcp{Change $Q$ table if necessary and update the trace segment}
    \Def{$updateStep(s,a,s')$}{
        \If{$\neg targetReached$}{
            $nextPred \gets arg \max_i pred_i(s')$ \;
            $reward \gets$ \leIf{$nextPred > curPred$}{$\top$}{$\bot$}
            $outOfSpace \gets$ \leIf{$nextPred \neq curPred$}{$\top$}{$\bot$}
            \If{$oneTime \land nextPred = n$}{
                $targetReached \gets \top$
            }
        }
        \Else{
            $reward \gets \bot$\;
            $outOfSpace \gets \bot$
        }
        $traceSegments_{curPred} \gets traceSegments_{curPred}.(s, a, s', reward, outOfSpace)$\;
        $curPred \gets nextPred$
    }
    \BlankLine

    \tcp{Update the corresponding $Q$-tables using the segments}
    \Def{$update(\_)$}{
        \For{$traceSegments_p, p = pred_1, \cdots, pred_n$}{
            \For{$(s,a,s',reward,outOfSpace) \in traceSegments_p$}{
                $t \leftarrow V_p(s,a) + 1$ \;
                $V_p(s,a) \leftarrow t$ \;
                $r \gets$ \leIf{$reward$}{$2+\frac{1}{t}$}{$\frac{1}{t}$}
                \eIf{$outOfSpace$}{
                    $m_{s'} = \max_a Q_p(s',a,0)$
                }{
                    $m_{s'} = \max_a Q_p(s',a,1)$
                }
                $Q_p(s,a) \leftarrow (1-\alpha).Q(s,a,1) + \alpha . max(r, \gamma.m_{s'})$
            }
        }
    }
    \caption{\biasExpAlgo{}: Biased exploration algorithm}
    \label{alg:\biasExpAlgo{}}
\end{algorithm}

==> contents/predh_general.tex <==
\begin{algorithm}[t]
    \SetAlgoLined
    \DontPrintSemicolon
    \SetKwInOut{Input}{Input}
    \Input{$K$, $H$, $E$, $predicates = \left\{pred_1, \cdots, pred_n\right\}, oneTime \in \left\{\top, \bot\right\}$}
    \BlankLine
    
    \For{$i = 1 \cdots n$}{
    	$ \pi_i.initialize() $ \;
    }
    \BlankLine

    \For{episode $k=1, \cdots, K$}{
        $state_1^k \gets E.reset()$ \;
        $trace^k \gets ()$ \;
        $ reached \gets \bot $ \;
        \For{step $h=1, \cdots, H$}{
        	\If{$reached = \bot$}{
        		$ p_h^k \gets activePredicate(predicates, state_h^k) $ \;
        		\If{$p_h^k = n \land oneTime = \top $}{
        			$ reached \gets \top $ \;
        		}
        	}
        	\Else{
        		$ p_h^k \gets n $ \;
        	}
        	\BlankLine
        	$ i \gets p_h^k $ \;
            $action_h^k \gets \pi_i^k.pick(state_h^k, E.actions(state_h^k))$ \;
            $state_{h+1}^k \gets E.step(action_h^k)$ \;
            $trace^k \gets append(trace^k, (state_h^k, action_h^k, state_{h+1}^k, p_h^k))$ \;
        }
        \For{$i = 1 \cdots n$}{
        	$\pi_i^{k+1} \gets \pi_i^k.update(trace^k)$ \;
        }
    }
    \BlankLine
    \caption{\biasExpAlgo{} - Biased exploration algorithm}
    \label{alg:predh_gen}
\end{algorithm}


==> contents/sys_model.tex <==
\section{A Primer on Reinforcement Learning and Q-Learning}
\label{sec:sys_model}

We introduced an RL agent, state space and action space in the earlier section. In this section we will define the terms more formally and use the definitions as a foundation when describing our contributions, the algorithms \pureExpAlgo{} and \biasExpAlgo{}.

An RL agent explores an unknown environment modelled as a Markov Decision Process (MDP). An MDP consists of the following components,
\begin{enumerate}
    \item A state space $\stateSpace$
    \item An action space $\actionSpace$
    \item An initial state $s_0 \in \stateSpace$
    \item A transition probability function $\mathcal{T}(s,a,s'): \stateSpace \times \actionSpace \times \stateSpace  \rightarrow [0,1]$ - $\mathcal{T}(s,a,s')$ indicates the probability of the transition $s \xrightarrow{a} s'$
    \item A reward function $\mathcal{R}: \stateSpace \times \actionSpace \times \stateSpace \rightarrow \mathbb{R}$ that specifies a reward for a specific transition
\end{enumerate}


\input{contents/generic_rl.tex}


Algorithm~\ref{alg:generic_rl} describes a generic Reinforcement Learning loop. The inputs are - number of iterations (or episodes $K$), number of steps for each iteration (horizon $H$), the environment being explored $E$ and an RL agent $A$. The environment behavior is captured by its functions - $reset$ to start a new episode from its initial state, $actions$ to return the available actions in the current state, and $step$ to transition in a new state according to the agent's picked action. 
Each iteration starts from the environment's initial state. At each step, the RL agent selects the next action, from the set of possible actions, according to its policy, and observes the resulting state and reward. Often, a discount factor $\gamma$ models the decaying value of rewards collected later on in the episode. We define some generic agent's functions that are called during the loop and allow for different specific implementations. Namely, $newEpisode$ at the beginning of each episode, $recordStep$ after each timestep, and $processEpisode$ at the end of the episode. For example, an agent implementation can use $newEpisode$ to reset its episode trace, $recordStep$ to append each transition, and then use the full trace to update its policy in $processEpisode$.  The goal of the RL agent is to maximize the expected reward collected throughout the episode, learning an optimal policy. To learn such a policy, the agent iteratively updates its own policy according to the observed transitions and rewards.

A popular RL algorithm is $Q$-Learning~\cite{DBLP:journals/ml/WatkinsD92}. In $Q$-Learning, the agent keeps an estimate $Q(s,a)$ of the expected reward for a given state ($s$) and action ($a$) pair called $Q$-value. For a given transition $(s,a,s')$, and its associated reward $r(s,a,s')$, $Q$-learning updates the Q-value as follows:
\[Q(s,a) = (1-\alpha) Q(s,a) + \alpha (r(s,a,s') + \gamma \max\limits_{a'} Q(s',a'))\]
where $\alpha, \gamma \in [0,1]$ are hyper-parameters representing the learning rate and discount factor respectively. Intuitively, each time the outcome of picking a state-action pair is observed, its $Q$-value is updated based on the observed reward and estimated value of the next state. $\alpha$ determines how quickly the $Q$-value changes at each update, while $\gamma$ defines how quickly delayed rewards decrease in value.

The collection of all the $Q$-Values (one for each $state-action$ pair) is often referred as $Q$-Table. The agent's policy follows the values in the $Q$-Table. At each step, given the current $state$ of the environment, the policy will pick actions based on how high is their $Q$-Value. In order to guarantee convergence to an optimal policy, all available actions should have non-zero probability to be picked.

Two common ways to pick actions are the following:
\begin{itemize}
    \item $\epsilon$-greedy - outputs the action with the highest $Q$-Value with probablility (1 - $\epsilon$), and a random action with probability $\epsilon$
    \item Softmax - outputs an action $a$ with probability proportional to its $Q$-Value: \\
     \[ p(a) = \frac{e^{Q(s,a)}}{\sum_{a'}e^{(Q(s,a'))}} \]
\end{itemize}

Exploration plays a major role in the RL agent learning performance. It improves efficiency in discovering hard-to-reach rewards and avoiding local optima. Common methods to incetivize the agent's exploration are:
\begin{itemize}
	\item Optimistic Initialization - $Q$-Values are initialized to positive values, the agent is incentivized to repeatedly explore each state-action pair, before its value eventually decays to 0
	\item Exploration Bonus - an explicit bonus that is added to the reward. It is usually a function of the number of visits, but it can depend on more complex metrics of novelty
\end{itemize}
In our work, exploration bonuses will be, with the exception of the rewards provided for biasing, the only source of rewards for the RL agent.

In Section~\ref{sec:transition_system}, we will describe our modelling of distributed systems as an environment.

==> overview.tex <==
\section{Overview}
\label{sec:overview}




A distributed system consists of a set of processes communicating with each other by sending and receiving messages. The state of each process consists of a set of variables that are modified when they send or receive messages. Combining the different states of the processes and including the messages in transit gives us the state of the entire system. A bug manifests when the system reaches a bad state. A naive approach to testing distributed systems can be to explore the state space randomly. Existing approaches such as Jepsen and PCTCP \Comment{Need ref} explore the state space more efficiently and improve the likelihood of reaching a buggy state. Our approach is to train a Reinforcement Learning (RL) agent to explore the state space. We build on existing work of using RL agents for Controlled Concurrency Testing (CCT)~\cite{DBLP:journals/pacmpl/MukherjeeDBL20} which has proven to be more effective in finding bugs and has better coverage than other approaches.

In CCT, we control the messages exchanged between processes and time of each process. A \emph{scheduler} is chosen to explore the state space. In each step, the \emph{scheduler} chooses an \emph{action} to perform. For example, choosing the next message to deliver. A random \emph{scheduler} will choose uniformly at random from the bag of messages. The state of the system together with the actions make up the testing \emph{environment}. We propose new \emph{schedulers} to test distributed systems and compare its effectiveness in exploration against existing random and other RL based \emph{schedulers}.

In this section, we will use different Grid \emph{environments} as running examples to visualize drawbacks of existing approaches and motivate our approach. Consider, for example, an environment of layered two dimensional grids, each of size $n\times n$. The state of the system consists of the layer number and the current position in the grid, i.e. $(l,x,y)$. Within each grid, the actions of the agent are to move up, down, left or right. Additionally, there are special positions in the state which act as doors to a grid to a higher layer. The agent can choose to go through the door as an action. For example, in a 3-layered $4\times4$ grid, $(1, 2, 2) \rightarrow (2, 3, 1)$ is a door.

The layered grid environment also serves as an analogy to the state space of the distributed systems. Moving across different positions in the same grid is similar to delivering different messages. However, akin to taking the doors, delivering a quorum of messages (for a successful commit) opens up a new section of the state space to be explored. Note that in the grid world doors only lead to higher grids and the action is irreversible. Similarly, in the distributed systems world a commit cannot be reverted.

Our contributions are the following: (1) we compare empirical performance of different algorithms for learning-based schedulers, (2) we analyse and discuss the importance of state abstractions in learning-based CCT, and (3) we propose a framework to bias testing towards specific executions.


\begin{figure}
	%\centering
	\includegraphics[scale=0.35]{images/grids_env.pdf} 
	\label{fig:grids_env}
\end{figure}

\subsection*{Different Reinforcement Learning exploration algorithms}
A learning-based scheduler, as proposed in ~\cite{DBLP:journals/pacmpl/MukherjeeDBL20}, works as an agent whose task is to explore a given environment (the system under test, in this case). At each exploration step, the scheduler observes a state of the environment, picks an action according to its policy and receives a reward. In this setting, the reward consists in an exploration bonus, having higher values for states that have been visited less times. The scheduler's policy is constantly updated, with the goal of maximizing rewards and hence maximize the environment exploration. The way the policy is updated depends on the internal Reinforcement Learning algorithm of the scheduler. In this case, Q-Learning ~\cite{DBLP:journals/ml/WatkinsD92} is used. In practice, Q-Learning keeps an estimation of each state-action pair expected reward, and picks actions accordingly.

To improve the exploration performance, we designed a different variant of the algorithm proposed in ~\cite{DBLP:journals/pacmpl/MukherjeeDBL20}. First, the reward is defined as a decreasing positive exploration bonus instead of a negative penalization. Second, updates use the maximum value among immediate reward and next state reward. This allows the algorithm to focus only on less explored states, ignoring how many times the states on the path to reach them have been visited. And third, the choice of actions is greedy with respect to their values. We show that this results in a better exploration performance in this setting.

To provide a visual intuition of the exploration performance of the algorithms, we use a two-dimensional grid environment. The goal of the algorithm is to explore, for a given episodes budget, as many different states of the environment as possible. This is conceptually analogous to maximizing the coverage of execution states of a system under test. 

The example environment is shown in figure \ref{fig:grid_15x4}, together with the algorithms exploration performance. Each tile of the grid is a state, with the color representing the exploration density. The tiles that are not displayed have not been explored by the scheduler. \emph{Random} represents the baseline random scheduler, where actions are chosen randomly, and no learning happens. As expected, \emph{Random} struggles to find states further away from the initial location, resulting in a poor exploration of the higher layer grids. \emph{Penalty} is the scheduler proposed in ~\cite{DBLP:journals/pacmpl/MukherjeeDBL20}. It is able to outperform the random baseline by repeatedly taking the door leading to higher layer grids. However, it is not able to fully explore the environment within the given budget, and the exploration does not appear to be uniform. For example, the corners of the first grid are visited more often. \emph{Bonus Max} shows the performance of our algorithm. Within the budget, it successfully explores the entire state space of the environment by exploiting the doors leading to higher layers grids. It is observable how the algorithm is repeatedly taking the paths that lead to higher layers grids.

In section \ref{sec:experiments}, we show that a similar performance gap is observable when using the same algorithms for learning-based controlled concurrency testing of distributed systems

\begin{figure}
	\centering
	\includegraphics[scale=0.35]{images/grids3Ds_env.pdf}
	\caption{grid\_15x4 environment, green tile represents the starting location, doors are shown as colored pairs of tiles, allowing to move from red to blue.
		Random, Penalty and Bonus Max show the exploration performance of the algorithms after 10000 episodes. Visible tiles have been visited at least once, the color is proportional to the number of visits (red means higher).
	}  
	\label{fig:grids3Ds_env}
\end{figure}

\begin{figure}
	\begin{subfigure}{.33\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{images/Multigrid_15x4_random.pdf}
		\caption{random}
		\label{fig:sfig1}
	\end{subfigure}%
	\begin{subfigure}{.33\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{images/Multigrid_15x4_penalty.pdf}
		\caption{penalty}
		\label{fig:sfig2}
	\end{subfigure}
	\begin{subfigure}{.33\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{images/Multigrid_15x4_bonusmax.pdf}
		\caption{bonusmax}
		\label{fig:sfig3}
	\end{subfigure}
	\caption{plots of....}
	\label{fig:2d_exploration}
\end{figure}

\subsection*{State abstractions}
Learning-based testing does not simply reduce to the choice of a learning algorithm. The scheduler explores the system as an environment, performing actions based on the observed states. For real-world systems, it is not feasible to provide the full system state to the scheduler. In fact, the scheduler will only observe a representation of the system state that is called a \emph{state abstraction}. A \emph{state abstraction} is a function that maps a system state into an abstract representation of it, omitting part of the information.

The state abstraction defines the state space for the scheduler to explore. The scheduler will consider two states to be different only if they are mapped into different abstracted states. As discussed in ~\cite{DBLP:journals/pacmpl/MukherjeeDBL20}, this plays a crucial role in the exploration performance. Moreover, the quality of a state abstraction is not absolute, but it strictly depends on the testing target coverage. Usually, when testing a system, only part of its state is relevant for finding bugs. Hence, the rest is omitted, and the resulting target state space is itself an abstraction of the original space. The number of states covered in this target space is the metric to evaluate the testing exploration performance and the quality of the chosen abstraction.

Imagine a system consisting into a set of nodes, each of them holding an internal value. A state of such system can be defined as a set of \emph{node id}, \emph{value} pairs. Whether to abstract away the \emph{node id} information from the state abstraction strictly depends on the target space. In general, it can be abstracted away to ignore redundant reorderings and only explore different values configurations for the set of nodes. However, in case the system logic requires to explore explicit combinations of \emph{node id}, \emph{value} pairs, it should be included in the abstraction. 

There are a couple of considerations relative to the choice of the state abstraction and the consequent exploration performance.

%(1): target coverage is not the optimal state abstraction
The first consideration is that the target state abstraction might not be the optimal choice for the scheduler. A natural solution could be to provide the scheduler with the target space as its state abstraction. Although this can be, in general, a reasonable choice, it might not be the optimal one. One such case is when the target abstraction is not capturing some of the system's dynamics. Imagine the same example shown in figure \ref{fig:grid_15x4}, and let us suppose that our target space is given by only the rows of each grid. If we provide the row coordinate as state abstraction to the scheduler, omitting the column, it will fail to recognize the position of the doors towards higher layer grids. Providing both rows and columns coordinates, even if not part of the target space, will result in a better exploration performance. 

In contrast, there can be inverse scenarios, where reducing the informativeness of the abstraction results in a better exploration performance. To show this, we use the three-dimensional grid environment shown in fig... In the example, the doors are replicated at each depth level of the cube, with their location depending only on the other two dimensions. In the plots (ref), we compare the exploration performance using the original space abstraction and a flattened abstraction ignoring the depth coordinate. The flattened abstraction, albeit not containing complete information of the target space, speeds up the exploration process and results in a better coverage.

%(2): choosing abstractions is hard/risky
The second consideration is that finding a good state abstraction is not trivial. Its design requires domain knowledge and effort, and it can lead to poor coverage results if unsuccessful. It might seem easy to design state abstractions for a grid environment, but it becomes more challenging when considering the execution space of a distributed system, where the actions are relative to the messages being delivered. In this more challenging setting, it is possible to end up designing bad state abstraction, resulting in a poor exploration performance. 

One such case is when the crucial states for the environment's dynamics are not captured by the abstraction (doors in the grid environment). The scheduler will be unable to recognize and exploit those states. Another case is when information required to avoid actions that are detrimental for exploration is abstracted away. For example, actions that are resetting some progress towards next states. To give a visual example of both these cases, consider the same environment in fig ... in two variants. In variant (A) the doors are located in the level with maximum depth in each cube. In variant (B) an action that resets the depth coordinate to zero is added. The flattened abstraction, that worked very well in the previous example, now performs poorly on exploration of both environment variants. For variant (A), fig ..., it fails to reach higher layer grids by not recognizing the doors, while for variant (B), fig ..., it fails to reach the deeper floors by not learning to avoid the reset action.

\subsection*{Biasing exploration}
Our main contribution is a framework to bias the environment exploration towards specific areas of the state space. It allows the scheduler to use a more informative abstraction while mitigating the problem of the state space size. In our tool? the tester can specify the exploration target subspace as a predicate over the state abstraction. Moreover, it can specify additional predicates to help the scheduler to reach the target subspace. Our learning-based scheduler will learn a policy to reach the target subspace and maximize its coverage.

This approach has several benefits. First, given a state abstraction and a target subspace, it enables the scheduler, when provided with the right sequence predicates, to explore the subspace more efficiently compared to the standard learning-based scheduler. Second, it does not require the state abstraction to be specific for the target subspace. It suffices to design a predicate sequence to efficiently explore of a target subspace, while using a general, informative, state abstraction. Third, it allows to preserve the informativeness of the state abstraction to improve the exploration of the target subspace. Designing a smart abstraction can also lead to a target subspace faster, but the information abstracted away might result in the drawbacks discussed before, reducing the exploration performance within the target subspace. 

Additionally, we argue that designing predicates to bias exploration requires less effort than designing state abstractions. In general, the predicates do not require operational knowledge of the system, it is sufficient to provide the properties of the target states and the learning algorithm will automatically learn how to reach those states. It also allows to incrementally build the predicate sequence if the scheduler is struggling to reach the target subspace within a given budget.

To visualize how our approach can overcome the difficulties encountered by the previously designed abstraction, we run again the scheduler on our grid examples. In fig. our scheduler, provided with a set of predicates corresponding to the the sequence of grids to reach the target one, is compared with the standard scheduler and the one using the flattened abstraction. Our scheduler efficiently explores the target subspace while working with the full state space abstraction. In fig . , we run the same experiment adding the reset depth action. In contrast with the flattened abstraction scheduler, our scheduler learns to avoid the reset action and is still able to explore the full depth of the grid.

In the last set of experiments, we show how our scheduler is flexible with respect to the input predicates. It is able to explore the target subspace with different set of predicates, including incomplete sequences of grids. All the schedulers provided with more than one predicate are able to explore the target grid with a significant lower budget than the one required by the standard scheduler. The scheduler provided with only the target subspace predicate fails to explore it within the budget, meaning that the target subspace requires additional intermediate predicates to speed up the exploration.


